An improved non-reflecting outlet boundary condition for weakly-compressible SPH

Implementation of an outlet boundary condition is challenging in the context of the weakly-compressible Smoothed Particle Hydrodynamics method. We perform a systematic numerical study of several of the available techniques for the outlet boundary condition. We propose a new hybrid approach that combines a characteristics-based method with a simpler frozen-particle (do-nothing) technique to accurately satisfy the outlet boundary condition in the context of wind-tunnel-like simulations. In addition, we suggest some improvements to the do-nothing approach. We introduce a new suite of test problems that make it possible to compare these techniques carefully. We then simulate the flow past a backward-facing step and circular cylinder. The proposed method allows us to obtain accurate results with an order of magnitude less particles than those presented in recent research. We provide a completely open source implementation and a reproducible manuscript.

==> figures/pulse2d_edac_test/pulse2d_edac_test_l2_u.tex <==
\begin{tabular}{lrrrr}
\toprule
        Methods & $\alpha = 0.1$ & $\alpha = 0.2$ & $\alpha = 0.5$ & $\alpha = 1.0$ \\
\midrule
 Characteristic &          0.063 &          0.060 &          0.057 &          0.055 \\
     Do-Nothing &          0.061 &          0.046 &          0.038 &          0.042 \\
         Hybrid &          0.038 &          0.038 &          0.035 &          0.034 \\
         Mirror &          0.125 &          0.112 &          0.106 &          0.105 \\
 New Do-Nothing &          0.070 &          0.055 &          0.042 &          0.050 \\
\bottomrule
\end{tabular}

